Quantum Group Actions

In quantum cryptography, there could be a new world, Microcrypt, where cryptography is possible but one-way functions (OWFs) do not exist. Although many fundamental primitives and useful applications have been found in Microcrypt, they lack ``OWFs-free'' concrete hardness assumptions on which they are based. In classical cryptography, many hardness assumptions on concrete mathematical problems have been introduced, such as the discrete logarithm (DL) problems or the decisional Diffie-Hellman (DDH) problems on concrete group structures related to finite fields or elliptic curves. They are then abstracted to generic hardness assumptions such as the DL and DDH assumptions over group actions. Finally, based on these generic assumptions, primitives and applications are constructed. The goal of the present paper is to introduce several abstracted generic hardness assumptions in Microcrypt, which could connect the concrete mathematical hardness assumptions with applications. Our assumptions are based on a quantum analogue of group actions. A group action is a tuple $(G,S,\star)$ of a group $G$, a set $S$, and an operation $\star:G\times S\to S$. We introduce a quantum analogue of group actions, which we call quantum group actions (QGAs), where $G$ is a set of unitary operators, $S$ is a set of states, and $\star$ is the application of a unitary on a state. By endowing QGAs with some reasonable hardness assumptions, we introduce a natural quantum analogue of the decisional Diffie-Hellman (DDH) assumption and pseudorandom group actions. Based on these assumptions, we construct classical-query pseudorandom function-like state generators (PRFSGs). Because classical group actions are instantiated with many concrete mathematical hardness assumptions, our QGAs could also have some concrete (even OWFs-free) instantiations.

==> construction_of_UCSG.tex <==


\section{Construction of (classical-query) Unclonable FSG}


% If the goal is UPSG instead of PRFSG, then we can weaken the PRSG-like assumption as QGA's unpredictability; 
% roughly speaking, the adversary cannot predict $g \ket{x}$ with $g \gets G$ and $\ket{x} \gets S$, while it is given $\ket{x}$. 
% There are two different flavors of definitions as one-wayness of QGA, depending on the description of $\ket{x}$. 

Our goal in this section is to construct a classical-query unclonable function-like state generator (UCFSG) from QGAs.
We first define the unclonability of QGA and study its implications. 
We then show that our NR-like FSG is a classical-query UCFSG if QGA is NR and unclonable. 

\subsection{Unclonable QGA} 
\begin{definition}[Unclonable QGA (UC QGA)] \label{def:Type-I-Unc}
A QGA $(G,S)$ is \emph{unclonable} if 
for any QPT adversary $\cA$ and any polynomials $t_0$ and $t$,
$\Pr[\top\gets\cC]\le\negl(\secp)$ is satisfied in the following security game.
\begin{enumerate}
    \item 
    The challenger $\cC$ chooses $\ket{s} \gets S$ and $g \gets G$. 
    \item
    $\cC$ sends $\ket{s}^{\otimes t_0}$ to $\cA$.
    $\cC$ also sends $(g\ket{s})^{\otimes t}$ to $\cA$. 
    \item 
    $\cA$ returns $\xi$, which is a quantum state on $t' > t$ registers $\mathbf{R}_1,\dots,\mathbf{R}_{t'}$. 
    \item 
    For $i \in [t']$, 
    $\cC$ projects the state on $\mathbf{R}_i$ onto $g \ket{s}$. 
    If at least $t + 1$ projection tests pass, then $\cC$ outputs $\top$. 
    Otherwise, it outputs $\bot$. 
\end{enumerate}
\end{definition}

% \xagawa{Does this directly imply private money? The first state $\ket{x}^{\otimes t}$ might be problematic.}
% \xagawa{Should we define Unclonable State Generator?}
% \xagawa{Maybe unclonable state generator = private money.}

It is easy to show that unclonability implies unpredictability. 
\begin{lemma} \label{lem:UC->UP}
If QGA is unclonable, then it is unpredictable. 
\end{lemma}
\begin{proof}
It is easy to construct a reduction algorithm $\cB$ as follows: 
\begin{enumerate}
\item $\cB$ is given $\ket{s}^{\otimes t}$ and $g\ket{s}$, where $\ket{s} \gets S$ and $g \gets G$. 
\item It runs $\cA$ on input $\ket{s}^{\otimes t}$ and obtains $\rho$. 
\item It outputs $\ket{\xi} = g \ket{s} \otimes \rho$. 
\end{enumerate}
\xagawa{Fill the rest.}
\end{proof}
%
% We also note that if $t$ is a constant, then unclonability implies one-wayness. 

We can show that the unclonability of QGA implies one-wayness, 
as Morimae and Yamakawa showed that private money with pure quantum money states implies a one-way state generator~\cite[Thm.5.4]{TQC:MorYam24}, 
\begin{lemma} \label{lem:UC->OW}
If QGA is unclonable, then it is one-way. 
\end{lemma} 
%\xagawa{Really? Should we amplify the success probability of A?}
%\xagawa{The proof is very similar to that for Pure-state private money and OWSG in \cite{TQC:MorYam24}.}
\begin{proof}
Suppose that QGA is not one-way; 
that is, that there exist 
a QPT adversary $\cA$ and two polynomials $t$ and $p$ satisfying, for infinitely often $\secp$, 
\[
\sum_{s,g,g'} \Pr[\ket{s} \gets S(1^\secp)] \cdot \Pr[g \gets G(1^\secp)] 
\cdot \Pr[g' \gets \cA(\ket{s}^{\otimes t} \otimes (g\ket{s})^{\otimes t})] 
\cdot \left\lvert \bra{s}(g')^\dagger g \ket{s} \right\rvert^2 \geq 1/p. 
\]
We define a set 
\[
\mathsf{Good} \coloneqq 
\left\{ (s,g,g') : \left\lvert \bra{s}(g')^\dagger g \ket{s} \right\rvert^2 \geq 1/2p 
\right\}. 
\]
We have 
\begin{align*}
1/p 
& \leq 
\sum_{s,g,g'} \Pr[\ket{s} \gets S(1^\secp)] \cdot \Pr[g \gets G(1^\secp)] 
\cdot \Pr[g' \gets \cA(\ket{s}^{\otimes t} \otimes (g\ket{s})^{\otimes t})] 
\cdot \left\lvert \bra{s}(g')^\dagger g \ket{s} \right\rvert^2 \\ 
&= 
\sum_{(s,g,g') \in \mathsf{Good}} \Pr[\ket{s} \gets S(1^\secp)] \cdot \Pr[g \gets G(1^\secp)] 
\cdot \Pr[g' \gets \cA(\ket{s}^{\otimes t} \otimes (g\ket{s})^{\otimes t})] 
\cdot \left\lvert \bra{s}(g')^\dagger g \ket{s} \right\rvert^2 \\ 
&\quad+\sum_{(s,g,g') \not\in \mathsf{Good}} \Pr[\ket{s} \gets S(1^\secp)] \cdot \Pr[g \gets G(1^\secp)] 
\cdot \Pr[g' \gets \cA(\ket{s}^{\otimes t} \otimes (g\ket{s})^{\otimes t})] 
\cdot \left\lvert \bra{s}(g')^\dagger g \ket{s} \right\rvert^2 \\ 
&< \sum_{(s,g,g') \in \mathsf{Good}} \Pr[\ket{s} \gets S(1^\secp)] \cdot \Pr[g \gets G(1^\secp)] 
\cdot \Pr[g' \gets \cA(\ket{s}^{\otimes t} \otimes (g\ket{s})^{\otimes t})] + 1/2p.
\end{align*}
Thus, we have 
\[
\sum_{(s,g,g') \in \mathsf{Good}} \Pr[\ket{s} \gets S(1^\secp)] \cdot \Pr[g \gets G(1^\secp)] \cdot \Pr[g' \gets \cA(\ket{s}^{\otimes t} \otimes (g\ket{s})^{\otimes t})] > 1/2p.
\]

Let $\ell$ be a polynomial specified later.
We construct a reduction algorithm $\cB$ against unclonability as follows: 
\begin{enumerate}
\item $\cB$ is given $\ket{x}^{\otimes (\ell + t)}$ and $(g\ket{x})^{\otimes t}$, where $\ket{x} \gets S$ and $g \gets G$. 
\item It runs $\cA$ on input $\ket{x}^{\otimes t}$ and $(g\ket{x})^{\otimes t}$ and obtains $g'$. 
\item $\cB$ outputs $\xi = (g'\ket{s})^{\otimes \ell}$ and halts. 
\end{enumerate}
Let $v_j$ be the bit that is set as $1$ if the projection test of $g'\ket{s}$ onto $g\ket{s}$ is $\top$. 
For any $(s,g,g') \in \mathsf{Good}$, we have 
\begin{align}
\Pr[v_j=1]
&= \Pr[\top \gets \mathsf{Proj}(g\ket{s}, g'\ket{s})] \nonumber \\
&\geq \Pr[\top \gets \mathsf{Proj}(g\ket{s}, g\ket{s})] - \sqrt{1-1/2p} \label{eq:rel2} \\ 
&= 1- \sqrt{1-1/2p} \geq 1/4p \label{eq:rel3} 
\end{align}
for any $j \in [\ell]$,
where \cref{eq:rel2} follows from the relation between the fidelity and the trace distance as discussed in~\cite[Footnote 19]{TQC:MorYam24}
 and \cref{eq:rel3} follows from the fact that $1 - x/2 \geq  \sqrt{1-x}$ for $x \in [0,1]$. 
We note that $\mathbb{E}[\sum_{j \in [\ell]} v_j] \geq \ell / 4 p$. 

Now, we adjust $\ell$ as $\max\{8p(t+1), 128p^2\}$. 
For any $(s,g,g') \in \mathsf{Good}$, we have 
\begin{align}
\Pr[\mathsf{Count}(g,s,(g'\ket{s})^{\otimes \ell}) \geq t + 1]
&= \Pr[\sum_{j \in [\ell]} v_j \geq t + 1] \geq \Pr[\sum_{j \in [\ell]} v_j \geq \ell/8p] \label{eq:bound1} \\ 
&= \Pr\left[\sum_{j \in [\ell]} v_j \geq \mathbb{E}[\sum_{j \in [\ell]} v_j] - \ell/8p\right] \label{eq:bound2} \\ 
&\geq 1 - \Pr\left[ \left\lvert \sum_{j \in [\ell]} v_j - \mathbb{E}[\sum_{j \in [\ell]} v_j] \right\rvert \geq \ell/8p\right] \nonumber \\
&\geq 1 - 2 \exp(-(\ell/8p)^2/\ell) = 1 - 2\exp(-\ell/64p^2) \label{eq:bound3} \\
&\geq 1 - 2e^{-2} \geq 1/2 \label{eq:bound4}, 
\end{align}
where we used $\ell \geq 8p (t+1)$ in \cref{eq:bound1}, $\mathbb{E}[\sum_{j \in [\ell]} v_j = 1] \geq \ell/4p$ in \cref{eq:bound2}, the Hoeffding inequality in \cref{eq:bound3}, and $\ell \geq 128p^2$ in \cref{eq:bound4}. 

Thus, $\cB$'s advantage is 
\begin{align*}
&\qquad \sum_{s,g,g'} \Pr[\ket{s} \gets S(1^\secp)] \cdot \Pr[g \gets G(1^\secp)] 
\cdot \Pr[g' \gets \cA(\ket{s}^{\otimes t} \otimes (g\ket{s})^{\otimes t})] 
\cdot \Pr[\mathsf{Count}(g,s,(g'\ket{s})^{\otimes \ell}) \geq t + 1] \\ 
&\leq \sum_{(s,g,g')\in \mathsf{Good}} \Pr[\ket{s} \gets S(1^\secp)] \cdot \Pr[g \gets G(1^\secp)] 
\cdot \Pr[g' \gets \cA(\ket{s}^{\otimes t} \otimes (g\ket{s})^{\otimes t})] 
\cdot \Pr[\mathsf{Count}(g,s,(g'\ket{s})^{\otimes \ell}) \geq t + 1] \\ 
&\leq \frac{1}{2} \sum_{(s,g,g')\in \mathsf{Good}} \Pr[\ket{s} \gets S(1^\secp)] \cdot \Pr[g \gets G(1^\secp)] 
\cdot \Pr[g' \gets \cA(\ket{s}^{\otimes t} \otimes (g\ket{s})^{\otimes t})] \\ 
&\leq \frac{1}{2} \cdot \frac{1}{2p} = 1/4p, 
\end{align*}
which is non-negligible for infinitely often $\secp$ as we wanted. 
\end{proof}

In addition, as a direct application, we can construct private money as follows: 
\begin{theorem} \label{thm:UC->PrivMon}
If QGA is unclonable, 
 then the following $(\KeyGen, \Mint, \Ver)$ is private money. 
\begin{itemize}
\item $\KeyGen(1^\secp) \to k$: 
Choose $\ket{x} \gets S$ and $g \gets G$. Output $k = (\ket{x},g)$. 
(Note that $\ket{x}$ is not a physical quantum state but its classical description). 
\item $\Mint(k) \to \ket{\$}$: Output $g\ket{x}$. 
\item $\Ver(k, \rho) \to \top/\bot$: Project $\rho$ onto $g\ket{x}$. If the projection test passes, then output $\top$. Otherwise, output $\bot$. 
\end{itemize}
\end{theorem}
The completeness is obvious. 

If private money is insecure, then there exists an adversary who receives $\ket{\$}^{\otimes t}$ for some polynomial $t=t(\secp)$ 
 and output $\xi$ that makes count outputs $\top$. 
Our adversary $\cB$ against UC QGA takes $\ket{x}$ and $(g \ket{x})^{\otimes t}$ as input, 
 passes $(g \ket{x})^{\otimes t}$ to $\cA$, and receives $\xi$ from $\cA$, and outputs $\xi$. 
If $\xi$ passes Count's test, then $\cA$ wins and $\cB$ wins. 
It is obvious that $\cB$'s simulation is perfect. 





% plus-one-secure MAC (m_^*1,\dots,m^*_{t}中のq+1個で検証が通る) -> unclonable MAC (m^*に対してt個タグを出してq+1個で検証が通る) ? 
% We need to simulate the oracle before declaring $m^*$... This is the problem... 
% plus-one-secure MAC -?-> EUF-CMA MAC 
% unclonable MAC -?-> EUF-CMA MAC ... ??? 
% EUF-CMA MAC -/-> unclonable MAC ... EUF-CMA MACで古典タグだとcloneし放題。量子タグの場合も古典タグを量子状態にしていると思うとclone可能？ OWFがないときのEUF-CMA MACを仮定しないといけない？



% \begin{definition}[Semi-Quanutm Unpredictable QGA] \label{def:Type-II-Unp}
% This is equivalent to type-I except that $\ket{x}^{\otimes t}$ that $\cC$ sends is replaced with its classical description.   
% \end{definition}
% \xagawa{This part will be filled after resolving the KeyGen distribution.}

% It is easy to see that a classical query UPSG implies an unpredictable QGA. 
% \begin{lemma} \label{thm:ccUPSG_UPQGA}
% If a classical query UPSG exists, then an unpredictable QGA exists. 
% \end{lemma}
% \begin{proof}
% Let $(\KeyGen,\Eval)$ be a UPSG and suppose that $\{0,1\}^n$ be a set of bit strings. 
% We construct a UP QGA as follows: 
% \begin{itemize}
% \item $\cG(1^\secp,k,\ket{\psi})$: 
% Let $U_k$ be a unitary such that $\ket{\phi_k(0^n)} = U_k \ket{0...0} = \Eval(k,0^n)$. Output $U_k$. 
% \item $\cS(1^\secp,j)$: Always output $\ket{0...0}$. 
% \end{itemize}

% We construct a reduction algorithm $\cB$ against the underlying UPSG by using an adversary against the UP QGA. 
% \begin{enumerate}
% \item $\cB$ is given $1^\secp$ from its challenger. 
% It prepares $\ket{0...0}^{\otimes t}$ and gives it to $\cA$. 
% \item $\cA$ returns $\rho$. $\cB$ returns $x^* = 0^n$ and $\rho$ and halts.
% \end{enumerate}
% The challenger of UPSG runs the projection test between $\rho$ and $\ket{\phi_k(x^*)} = \ket{\phi_k(0^n)} = U_k\ket{0...0}$, where $k \gets \KeyGen(1^\secp)$. 
% Hence, $\cB$ simulates $\cA$'s game perfectly. 
% If $\cA$ wins its game, then its projection test of $\rho$ with $U_k \ket{0...0} = \ket{\phi_k(0^n)}$ passes. 
% Thus, if $\cA$ wins, then $\cB$ also wins its game. This completes the proof. 
% \end{proof}







\subsection{Construction}

We can show that $(\KeyGen,\StateGen)$ in \cref{thm:PRNR->PRFSG} is unclonable if QGA is NR and unclonable. Roughly speaking, we consider $\mathsf{Real} = \mathsf{Game}_0$ and $\mathsf{Hybrid} = \mathsf{Game}_{\ell}$ as in the proof for \cref{thm:PRNR->PRFSG}. 
By using hybrid games, these games are computationally indistinguishable if QGA is NR. 
To win in $\mathsf{Hybrid} = \mathsf{Game}_\ell$, the adversary should output $\xi$ that makes projection tests pass at least $t+1$-times with respect to $h_{Q+1} \ket{s_0}$. This can be reduced to the unclonability of QGA. 
%, we construct a UCFSG as follows:
\begin{theorem} \label{thm:UCNR->UCFSG}
If NR QGA is unclonable, 
 then $(\KeyGen, \StateGen)$ in \cref{thm:PRNR->PRFSG} is a UCFSG. 
\end{theorem}
\begin{proof}
We define the following hybrid games $\mathsf{Game}_j$ for $j = 0,\dots,\ell$: 
\begin{enumerate}
\item 
The challenger samples $g_0 \gets G$ and $g_i \gets G$ for $i \in [j+1,\ell]$ and runs the adversary. 
\item 
Let $q$-th adversary's query be $x_q = (x_q[1],\dots,x_q[\ell]) \in \{0,1\}^\ell$. The challenger returns a quantum state $\ket{f_{j,q}}$ defined as follows: 
\begin{itemize}
\item If $j = 0$, then the challenger let $\ket{y_q} = g_0 \ket{s_0}$; 
\item Otherwise
\begin{itemize}
    \item if there exists $q' < q$ satisfying $(x_q[1],\dots,x_q[j]) = (x_{q'}[1],\dots,x_{q'}[j])$, then $\ket{y_q} = \ket{y_{q'}}$; 
    \item otherwise, it samples $g_q \gets G$ and $\ket{y_q} \coloneqq g_q \ket{s_0}$. 
\end{itemize}
\item Return $\ket{f_{j,q}} \coloneqq g_\ell^{x_q[\ell]} \cdots g_{j+1}^{x_q[j+1]} \ket{y_q}$. 
\end{itemize}
\item The adversary outputs $x^*$. 
If $x^* \in \{x_q\}_{q\in[Q]}$, then the adversary loses. 
\item Otherwise, the challenger generates $\ket{f_{j,{Q+1}}}^{\otimes t}$, where $\ket{f_{j,{Q+1}}}$ is the quantum state for the $Q+1$-th query $x^*$ defined in the above, and gives it to the adversary. 
\item The adversary outputs $\xi$ over the registers $\mathbf{R}_1,\dots,\mathbf{R}_{t'}$. 
For $i \in [t']$, $\cC$ projects $\rho$ onto $\ket{f_{j,Q+1}}$. If at least $t+1$ projection tests pass, then $\cC$ outputs $\top$. Otherwise, it outputs $\bot$. 
\end{enumerate}
It is easy to verify that $\mathsf{Game}_0$ is the original UPSG game.
Claim~\ref{claim:PRFS-hybrid} shows that $\mathsf{Game}_0 \approx_c \mathsf{Game}_1 \approx_c \dots \approx_c \mathsf{Game}_\ell$ if QGA is NR-like by considering $Q+1$ queries. 

Thus, we just need to bound the winning probability in $\mathsf{Game}_\ell$. 
In the game $\mathsf{Game}_{\ell}$, all the answers $\ket{f_{j,q}}$ are computed as $g_q \ket{s_0}$ for $q=1,\dots,Q+1$.
%with non-negligible probability while it has no knowledge of $h_{Q+1} \gets G$.
The following claim shows that the unclonability of QGA implies
that any QPT adversary cannot output $\xi$ that makes the projection test succeed at least $t+1$ times. 
\end{proof}
% \xagawa{If we use the PRSG assumption, the last statement is obvious. If not, we need an assumption.}
\begin{claim} 
$\Pr[\top \gets \mathsf{Game}_\ell]$ is negligible if QGA is unpredictable for $t_0 = Q$. 
\end{claim}
\begin{proof}
The reduction algorithm $\cB$ works as follows: 
\begin{enumerate}
\item $\cB$ is given $\ket{s}^{\otimes Q}$ and $(g \ket{s})^{\otimes t}$, where $\ket{s} \gets S$. It runs $\cA$. 
\item Let $x_q$ be the $q$-th query. If there exists $q' < q$ such that $x_q = x_{q'}$, then it returns $h_{q'} \ket{x}$. Otherwise, it samples $h_{q} \gets G$ and returns $h_{q} \ket{s}$. 
\item $\cA$ outputs $x^*$. If $x^* \in \{x_q\}_{q\in[Q]}$, then $\cB$ outputs $\bot$. 
\item Otherwise, $\cB$ gives $(g\ket{s})^{\otimes t}$ to $\cA$. 
\item Finally $\cA$ outputs $\xi$. $\cB$ also outputs $\xi$ to its challenger and halts. 
\end{enumerate}
This $\cB$ perfectly simulates $\mathsf{Game}_\ell$. Thus, $\cA$'s advantage is equal to $\cB$'s advantage. This completes the proof. 
\end{proof}


It is easy to construct an unclonable MAC from UCFSG. 
\begin{itemize}
\item $\KeyGen'(1^\secp) \to k$: This is $\KeyGen$ in \cref{thm:PRNR->PRFSG}. 
\item $\Tag(k, x) \to \tau$: Output $\ket{\phi_k(x)} = \StateGen(k,x)$ defined in \cref{thm:PRNR->PRFSG}.  
\item $\Ver(k, x, \rho) \to \top/\bot$: Generate $\ket{\phi_k(x)} = \StateGen(k,x)$. 
Project $\rho$ onto $\ket{\phi_k(x)}$. If the projection test passes, then output $\top$. Otherwise, output $\bot$. 
\end{itemize}







% \subsection{Quantum-Query UCFSG}

% Following the idea in the case of PRF (\cite{FOCS:Zhandry12}) again, we construct new UCFSG as follows: 
% Let $N = 2^\ell$. 
% The key space of new UCFSG is $K' = G^{\ell+1} \times P$, where $P$ is a set of primes in $(2^{\ell-1},2^{\ell}]$.
% The new domain is $X' = \{0,1\}^{2\ell+3}$ ($2^{2\ell+3} > 4 \cdot 2^{2\ell}$). 
% We treat $X'$ as $[8N^2]$. 

% \begin{claim}
% If UCFSG is classical-query secure then the new UCFSG is also. 
% \end{claim}
% \begin{claim}
% If UCFSG is quantum-query secure, then the new UCFSG is not. 
% \end{claim}
% \begin{proof}
% If UCFSG is quantum-query secure, then we can extract a period $a$ by using the Boneh-Lipton algorithm \emph{without querying $0$.} 
% \xagawa{Need to analyze the Boneh-Lipton algorithm... }
% We then query $a$ and $2a$ to the oracle and obtain $\ket{\phi_k(a)}$ and $\ket{\phi_k(2a)}$.  
% We declare $x^* = 0$ and obtain $\ket{\phi_k(0)}$. 
% We then output $\xi = \ket{\phi_k(a)} \otimes \ket{\phi_k(2a)}$. 
% Since $\ket{\phi_k(a)} = \ket{\phi_k(2a)} = \ket{\phi_k(0)}$, we succeed to clone the state. 
% \end{proof}


==> construction_of_UPSG.tex <==


\section{Construction of (classical-query) Unpredictable FSG}

If the goal is UPSG instead of PRFSG, then we can weaken the PRSG-like assumption as QGA's unpredictability; 
roughly speaking, the adversary cannot predict $g \ket{x}$ with $g \gets G$ and $\ket{x} \gets S$, while it is given $\ket{x}$. 
There are two different flavors of definitions as one-wayness of QGA, depending on the description of $\ket{x}$. 




\subsection{Unpredictable QGA} 
%\begin{definition}[Fully-Quantum Unpredictable QGA] \label{def:Type-I-Unp}
\begin{definition}[Unpredictable QGA (UP QGA)] \label{def:Type-I-Unp}
A QGA $(G,S)$ is unpredictable if 
for any QPT adversary $\cA$ and any polynomial $t$,
$\Pr[\top\gets\cC]\le\negl(\secp)$ is satisfied in the following security game.
\begin{enumerate}
    \item 
    The challenger $\cC$ chooses $\ket{s} \gets S$ and $g \gets G$. 
    \item
    $\cC$ sends $\ket{s}^{\otimes t}$ to $\cA$.
    \item 
    $\cA$ returns $\rho$.
    \item 
    $\cC$ projects $\rho$ onto $g \ket{s}$.
    If the projection is successful,
    $\cC$ outputs $\top$. Otherwise, it outputs $\bot$.
\end{enumerate}
\end{definition}
% \begin{definition}[Semi-Quanutm Unpredictable QGA] \label{def:Type-II-Unp}
% This is equivalent to type-I except that $\ket{x}^{\otimes t}$ that $\cC$ sends is replaced with its classical description.   
% \end{definition}
% \xagawa{This part will be filled after resolving the KeyGen distribution.}

It is easy to see that a classical query UPSG implies an unpredictable QGA. 
\begin{lemma} \label{thm:cqUPSG_UPQGA}
If a classical query UPSG exists, then an unpredictable QGA exists. 
\end{lemma}
\begin{proof}
Let $(\KeyGen,\Eval)$ be a UPSG and suppose that $\{0,1\}^\ell$ be a set of bit strings. 
We construct a UP QGA as follows: 
\begin{itemize}
\item $\cG(1^\secp,k,\ket{\psi})$: 
Let $U_k$ be a unitary such that $\ket{\phi_k(0^\ell)} = U_k \ket{0...0} = \Eval(k,0^\ell)$. Output $U_k$. 
\item $\cS(1^\secp,j)$: Always output $\ket{0...0}$. 
\end{itemize}

We construct a reduction algorithm $\cB$ against the underlying UPSG by using an adversary against the UP QGA. 
\begin{enumerate}
\item $\cB$ is given $1^\secp$ from its challenger. 
It prepares $\ket{0...0}^{\otimes t}$ and gives it to $\cA$. 
\item $\cA$ returns $\rho$. $\cB$ returns $x^* = 0^\ell$ and $\rho$ and halts.
\end{enumerate}
The challenger of UPSG runs the projection test between $\rho$ and $\ket{\phi_k(x^*)} = \ket{\phi_k(0^\ell)} = U_k\ket{0...0}$, where $k \gets \KeyGen(1^\secp)$. 
Hence, $\cB$ simulates $\cA$'s game perfectly. 
If $\cA$ wins its game, then its projection test of $\rho$ with $U_k \ket{0...0} = \ket{\phi_k(0^\ell)}$ passes. 
Thus, if $\cA$ wins, then $\cB$ also wins its game. This completes the proof. 
\end{proof}

% It is also easy to check if OW QGA is UP QGA; ??? 
% the reduction algorithm takes $\ket{s}^{\otimes (t+1)}$ and $(g \ket{s})^{\otimes (t+1)}$, runs an adversary against UP QGA on input $\ket{s}^{\otimes t}$, receives and $\rho$, and outputs $\rho \coloneqq g' \ket{s}$. 






\subsection{Construction}


If NR QGA is unpredictable, then our construction is UPSG. 
\begin{theorem} \label{thm:UPNR->UPFSG}
$(\KeyGen,\StateGen)$ in \cref{thm:PRNR->PRFSG} is classical-query UPSG 
if NR QGA is unpredictable. 
\end{theorem}
\begin{proof}
We define the following hybrid games $\mathsf{Game}_j$ for $j = 0,\dots,\ell$: 
\begin{itemize}
\item 
The challenger samples $g_0 \gets G$ and $g_i \gets G$ for $i \in [j+1,\ell]$ and runs the adversary. 
\item 
Let $q$-th adversary's query be $x_q = (x_q[1],\dots,x_q[\ell]) \in \{0,1\}^\ell$. The challenger returns a quantum state $\ket{f_{j,q}}$ defined as follows: 
\begin{itemize}
\item If $j = 0$, then the challenger let $\ket{y_q} = g_0 \ket{s_0}$; 
\item Otherwise
\begin{itemize}
    \item if there exists $q' < q$ satisfying $(x_q[1],\dots,x_q[j]) = (x_{q'}[1],\dots,x_{q'}[j])$, then $\ket{y_q} = \ket{y_{q'}}$; 
    \item otherwise, it samples $g_q \gets G$ and $\ket{y_q} \coloneqq g_q \ket{s_0}$. 
\end{itemize}
\item Return $\ket{f_{j,q}} \coloneqq g_\ell^{x_q[\ell]} \cdots g_{j+1}^{x_q[j+1]} \ket{y_q}$. 
\end{itemize}
\item Finally, the adversary outputs $x^*$ and a quantum state $\rho$. 
If $x^* \in \{x_q \}_{q\in[Q]}$, then the adversary loses. 
Otherwise, the challenger projects $\rho$ onto $\ket{f_{j,Q+1}}$, where $\ket{f_{j,Q+1}}$ is the answer for $x^*$. If the projection is successful, then the adversary wins. Otherwise, it loses. 
\end{itemize}
It is easy to verify that $\mathsf{Game}_0$ is the original UPSG game.
Claim~\ref{claim:PRFS-hybrid} shows that $\mathsf{Game}_0 \approx_c \mathsf{Game}_1 \approx_c \dots \approx_c \mathsf{Game}_\ell$ if QGA is NR-like by considering $Q+1$ queries. 
Thus, we just need to bound the winning probability in $\mathsf{Game}_\ell$. 
All the answer $\ket{f_{j,q}}$ are computed as $g_q \ket{s_0}$ (with consistency) for $q =1,\dots,Q+1$. This means that the adversary should output $\rho$ that makes the projection test succeed with non-negligible probability while it has no knowledge of $h_{Q+1} \gets G$.
The following claim shows that the unpredictability of QGA says that this should not hold. 
\end{proof}
% \xagawa{If we use the PRSG assumption, the last statement is obvious. If not, we need an assumption.}
\begin{claim} 
$\Pr[\top \gets \mathsf{Game}_\ell]$ is negligible if QGA is unpredictable with $t = Q$. 
\end{claim}
\begin{proof}
The reduction algorithm $\cB$ works as follows: 
\begin{enumerate}
\item $\cB$ is given $\ket{s}^{\otimes Q}$, where $\ket{s} \gets S$. It runs $\cA$. 
\item Let $x_q$ be the $q$-th query. If there exists $q' < q$ such that $x_q = x_{q'}$, then it returns $h_{q'} \ket{s}$. Otherwise, it samples $h_{q} \gets G$ and returns $h_{q} \ket{s}$. 
\item If $\cA$ outputs $\rho$, then $\cB$ outputs $\rho$ and halts. 
\end{enumerate}
This $\cB$ perfectly simulates $\mathsf{Game}_\ell$. Thus, $\cA$'s advantage against UP QGA is equal to $\cB$'s advantage. This completes the proof. 
\end{proof}
% \begin{claim} 
% $\Pr[\top \gets \mathsf{Game}_\ell]$ is negligible if QGA is semi-quantum unpredictable.
% \end{claim}
% The proof is essentially the same as the above except that $\cB$ can produce $\ket{x}$ from its classical description. 




% \subsection{Quantum-Query UPFSG}

% Following the idea in the case of PRF (\cite{FOCS:Zhandry12}) again, we construct new UPFSG as follows: 
% Let $N = 2^\ell$. 
% The key space of new UPFSG is $K' = G^{\ell+1} \times P$, where $P$ is a set of primes in $(2^{\ell-1},2^{\ell}]$.
% The new domain is $X' = \{0,1\}^{2\ell+3}$ ($2^{2\ell+3} > 4 \cdot 2^{2\ell}$). 
% We treat $X'$ as $[8N^2]$. 

% \begin{claim}
% If UPFSG is classical-query secure then the new UPFSG is also. 
% \end{claim}
% \begin{claim}
% If UPFSG is quantum-query secure, then the new UPFSG is not. 
% \end{claim}
% If UPFSG is quantum-query secure, then we can extract a period $a$ by using the Boneh-Lipton algorithm even without querying $0$. 
% We then query $a$ to the oracle and obtain $\ket{\phi_k(a)}$. 
% Finally, we output $x^* = 0$ and $\ket{\phi_k(a)}$. 


==> figure-relations_20240814.tex <==

\begin{figure}
\centering
\footnotesize
\begin{tikzpicture}[scale=0.7,%
triv/.style={thick,draw=black!70,->,dashed},]
%
\node (PRU)     at (  2,14) {PRU} ;
\node (cqPRFSG) at ( -2,10) {cqPRFSG} ;
\node (qqPRFSG) at (  2,12) {qqPRFSG} ;
\node (PRSG)    at ( -5, 8) {PRSG} ;
\node (cqUPSG)  at ( -2, 5) {cqUPSG} ;
\node (qqUPSG)  at (  2, 7) {qqUPSG} ;
\node (SKE)     at (  6, 2) {IND-CPA SKE} ;
\node (SKE+MAC) at (  2, 4) {\shortstack[c]{IND-CPA SKE \\ + EUF-CMA MAC}} ;
\node (MAC)     at ( -2, 1) {EUF-CMA MAC} ;
\node (ucMAC)   at (  2, 2) {Unclonable MAC} ;
\node (PrivMon) at (  2,-1) {Private Money} ; 
\node (OWSG)    at (  2,-3) {OWSG} ; 
\node (EFI)     at (  2,-5) {EFI} ; 
%
\node (PRDHQGA) at (-11,13) {PR+HaarPR+DDH QGA} ;
\node (PRNRQGA) at (-11,11) {PR+NR QGA} ;
\node (PRQGA)   at (-11, 8) {PR QGA} ;
\node (UPNRQGA) at (-14, 6) {UP+NR QGA} ;
\node (UPQGA)   at (-14, 3) {UP QGA} ;
\node (UCNRQGA) at ( -7, 3) {UC+NR QGA} ;
\node (UCQGA)   at ( -7, 0) {UC QGA} ;
\node (OWQGA)   at ( -7,-3) {OW QGA} ;
%
\draw[triv] ([xshift=-20pt] qqPRFSG.south) to node [above,midway] {} ([xshift=-20pt] cqPRFSG.north east);
\draw[triv] ([xshift=-20pt] qqUPSG.south)  to node [above,midway] {} ([xshift=-20pt] cqUPSG.north east);
\draw[triv] (cqPRFSG) to node [above,midway] {} (PRSG); 
\draw[triv] (ucMAC)   to node [right,midway] {} (PrivMon);
\draw[triv] (SKE+MAC) to node [right,midway] {} (SKE);
\draw[triv] (SKE+MAC) to node [right,midway] {} (MAC);
\draw[triv] (ucMAC)   to node [right,midway] {} ([xshift=-10pt] MAC.north east);
\draw[triv] (cqUPSG)  to node [right,midway] {} (MAC);
\draw[triv] (cqUPSG)  to node {OK} (0,3.5) to (0,-1.5) to (OWSG);
%\draw[thin,->] (cqPRFSG) to [bend left] node [right,midway] {\cite{C:AnaQiaYue22}}  (SKE); 
\draw[thick,->] (PRU)     to node [right,midway] {\cite{TCC:AGQY22}} (qqPRFSG); 
\draw[thick,->] (cqPRFSG) to [bend left=10] node [right,pos=.25] {\cite{C:AnaQiaYue22}*} ([xshift=-10pt] SKE+MAC.north); 
\draw[thick,->] (qqPRFSG) to node [right,midway] {\cite{EPRINT:MorYamYam24}} (qqUPSG); 
\draw[thick,->] (cqPRFSG) to node [left ,midway] {\cite{EPRINT:MorYamYam24}} (cqUPSG); 
\draw[thick,->] (SKE+MAC) to node [right,midway] {\cite{EPRINT:MorYamYam24}} (ucMAC); 
\draw[thick,->] (qqUPSG)  to node [right,midway] {\cite{EPRINT:MorYamYam24}} (SKE+MAC); 
\draw[thick,->,dotted] (PrivMon) to node [right,midway] {\cite{TQC:MorYam24}}  (OWSG); 
\draw[thick,->] (SKE) to [bend left] node [left,pos=.3] {\cite{TQC:MorYam24}} (OWSG.east); 
\draw[thick,->] (SKE) to [bend left=35] node [right,midway] {\cite{TQC:MorYam24}} (EFI.east); 
\draw[thick,->,dotted] (OWSG)    to node [right,midway] {\cite{STOC:KhuTom24}}  (EFI); 
\draw[thick,->] (PRSG) to node [left,pos=.1] {\cite{C:JiLiuSon18}} (-5,1) to (PrivMon); %[out=270,in=180] (PrivMon.west); 
%\draw[thin,->] (cqPRFSG) to [bend left] node [right,midway] {\cite{TCC:AGQY22}} (oTCCSKE); 
%
\draw[triv] (PRNRQGA) to node [right,midway] {}  (PRQGA); 
\draw[triv] (PRNRQGA) to node [left ,midway] {}  (UPNRQGA); 
\draw[triv] (PRQGA)   to node [left ,midway] {}  (UPQGA);
\draw[triv] (PRNRQGA) to node [left ,midway] {?} (UCNRQGA); 
\draw[triv] (PRQGA)   to node [left ,midway] {?} (UCQGA);
\draw[triv] (UPNRQGA) to node [left ,midway] {}  (UPQGA);
\draw[triv] (UCNRQGA) to node [left, midway] {}  (UCQGA);
\draw[triv] (UCQGA)   to node [left, midway] {OK}(OWQGA);
\draw[triv] (UCQGA)   to node [left, midway] {??}(PrivMon); 
%\draw[triv] (UPQGA)   to node [right,midway] {??}(OWQGA);
%
\draw[thin ,red,->] ([xshift=-10pt] cqPRFSG.north east) to node [below,midway] {x} ([xshift=-10pt] qqPRFSG.south); 
\draw[thin ,red,->] ([xshift=-10pt] cqUPSG.north east)  to node [below,midway] {x?}([xshift=-10pt] qqUPSG.south);
% \draw[thin ,red,->] (MAC)     to node [below,midway] {x?} (ucMAC); 
\draw[very thick,red,->] (PRDHQGA) to node [right,midway] {\cref{lemma-for-PRFS}} (PRNRQGA); 
\draw[very thick,red,<->] (PRSG)   to node [above,midway] {\cref{thm:PRSG_PRQGA}} (PRQGA);
\draw[very thick,red,->] (PRNRQGA) to node [above,midway] {\cref{theorem:PRFS}} (cqPRFSG);
\draw[very thick,red,->] (UPNRQGA) to node [above,midway] {\cref{theorem:UPSG}} (cqUPSG);
\draw[very thick,red,->] (UCNRQGA) to node [above,midway] {\cref{theorem:ucMAC}} (ucMAC); 
\draw[very thick,red,->] (cqUPSG)  to node [above,pos=.8] {\cref{thm:cqUPSG_UPQGA}} (UPQGA);
\draw[very thick,red,<->,dotted] (OWQGA) to node [above,midway] {\cref{thm:OWSG_OWQGA}} (OWSG);
\end{tikzpicture}
\caption{Relations. "cq" and "qq" denote classical-query and quantum-query. 
A gray thin arrow from primitive A to primitive B represents that primitive A trivially implies primitive B. 
A dotted arrow from primitive A to primitive B represents that primitive A with pure outputs implies primitive B.
*: \cite{C:AnaQiaYue22} shows that cqPRFSG implies IND-CPA SKE. Combined with cqUPSG implies EUF-CMA MAC, cqPRFSG implies IND-CPA SKE + EUF-CMA MAC. 
}
\label{fig:relations}
\end{figure}



% plus-one-secure MAC (m_^*1,\dots,m^*_{t}中のq+1個で検証が通る) -> unclonable MAC (m^*に対してt個タグを出してq+1個で検証が通る) ? 
% We need to simulate the oracle before declaring $m^*$... This is the problem... 
% plus-one-secure MAC -?-> EUF-CMA MAC 
% unclonable MAC -?-> EUF-CMA MAC ... ??? 
% EUF-CMA MAC -/-> unclonable MAC ... EUF-CMA MACで古典タグだとcloneし放題。量子タグの場合も古典タグを量子状態にしていると思うとclone可能？ OWFがないときのEUF-CMA MACを仮定しないといけない？



==> figure-relations_20240918.tex <==

\begin{figure}
\centering
%\footnotesize
\ifnum\fullpage=0
\tiny
\begin{tikzpicture}[scale=0.45,%
triv/.style={thick,draw=black!60,->,dashed},
open/.style={thick,blue,->},
ours/.style={thin,draw=red,->,double},
]
\else 
\footnotesize
\begin{tikzpicture}[scale=0.6,%
triv/.style={thick,draw=black!60,->,dashed},
open/.style={thick,blue,->},
ours/.style={thin,draw=red,->,double},
]
\fi 
%
\node at (  9,20) {\underline{qq primitives}};
\node at (  4,20) {\underline{cq primitives}};
\node at ( -2,20) {\underline{no-query primitives}};
\node at ( -8,20) {\underline{QGAs}};
\node at (-14,20) {\underline{NR QGAs}};
%
\node (OWF)     at (  0,18) {OWF} ;
\node (PRU)     at (  9,16) {PRU} ;
\node (qqPRFSG) at (  9,13) {qqPRFSG} ;
\node (cqPRFSG) at (  4,12) {cqPRFSG} ;
\node (qqUCFSG) at (  9,10) {qqUCFSG} ;
\node (cqUCFSG) at (  4, 9) {cqUCFSG} ;
\node (qqUPSG)  at (  9, 7) {qqUPFSG} ;
\node (cqUPSG)  at (  4, 6) {cqUPFSG} ;
\node (SKE)     at (  9, 1) {qmSKE} ;
\node (QPOTP)   at (  1,-1) {QPOTP} ;
\node (SKE+MAC) at (  9, 4) {qmSKE+cqMAC} ;
\node (ucMAC)   at (  4, 3) {UC MAC} ;
\node (MAC)     at (  4, 0) {cqMAC} ;
\node (PRSG)    at ( -4, 4) {PRSG} ;
\node (PrivMon) at ( -4, 1) {Private Money} ; 
\node (OWSG)    at (-1.5,-2) {OWSG} ; 
\node (EFI)     at (-1.5,-5) {EFI} ; 
% \node (UPSG)    at ( -4,-2) {UPSG} ; 
% \node (otSKE)   at (  4,-3) {otSKE} ;
%
\node (PRDHQGA) at (-14,16) {PR+HaarPR+DDH QGA} ;
\node (PRNRQGA) at (-14,13) {PR+NR QGA} ;
\node (PRQGA)   at ( -9, 5) {PR QGA} ;
\node (UCNRQGA) at (-14,10) {UC+NR QGA} ;
\node (UCQGA)   at ( -9, 2) {UC QGA} ;
\node (UPNRQGA) at (-14, 7) {UP+NR QGA} ;
\node (UPQGA)   at ( -9,-1) {UP QGA} ;
\node (OWQGA)   at (-6.5,-1) {OW QGA} ;
%
\draw[triv] ([yshift=10pt] qqPRFSG.south west) to node [above,midway] {} ([yshift=0pt] cqPRFSG.north east);
\draw[triv] ([yshift=10pt] qqUCFSG.south west) to node [above,midway] {} ([yshift=0pt] cqUCFSG.north east);
\draw[triv] ([yshift=10pt]  qqUPSG.south west) to node [above,midway] {} ([yshift=0pt]  cqUPSG.north east);
\draw[triv] (qqPRFSG) to node [above,midway] {} (qqUCFSG);
\draw[triv] (cqPRFSG) to node [above,midway] {} (cqUCFSG);
\draw[triv] (qqUCFSG) to node [above,midway] {} (qqUPSG);
\draw[triv] (cqUCFSG) to node [above,midway] {} (cqUPSG);
\draw[triv] (cqUCFSG) to [bend left=50] node [above,midway] {} (ucMAC);
\draw[triv] (cqPRFSG) to node [above,midway] {} (PRSG); 
\draw[triv] (cqUCFSG) to node [above,midway] {} (PrivMon);
% \draw[triv] (cqUPSG)  to node [above,midway] {} (UPSG); 
\draw[triv] (ucMAC)   to node [right,midway] {} (PrivMon);
\draw[triv] (SKE+MAC) to node [right,midway] {} (SKE);
\draw[triv] (SKE+MAC) to node [right,midway] {} (MAC.north east);
\draw[triv] (SKE)     to [bend left=20] node [right,midway] {} (QPOTP);
\draw[triv] (ucMAC)   to node [right,midway] {} (MAC);
\draw[triv] (cqUPSG)  to [bend right=45] node [left,midway] {} (MAC);
% \draw[triv] (PrivMon) to node [right,midway] {} (UPSG);
% \draw[triv] (QPOTP)   to node [right,midway] {} (otSKE);
%\draw[triv] (SKE)     to node [right,midway] {} (otSKE);
%
\draw[thick,->] ([yshift=10pt] PRU.west) -- coordinate (m) (OWF.east) node [above,midway] {\cite{Kre21}}; 
\draw[thick,shift={(m)}](-0.2,-0.1)--(0.2,+0.1);
\draw[thick,->] ([yshift=-10pt] OWF.east)     to node [below,midway] {\cite{HuangMa}} (PRU.west); 
% \draw[thick,->] (OWF.south)     to node [left,midway] {\cite{TCC:AGQY22}} (qqPRFSG); 
\draw[thick,->] (PRU)     to node [right,midway] {\cite{TCC:AGQY22}} (qqPRFSG); 
\draw[thick,->] (cqPRFSG) to node [right,pos=.1] {\cite{C:AnaQiaYue22}*} ([xshift=-10pt] SKE+MAC.north); 
\draw[thick,->] (SKE+MAC) to node [above,midway] {\cite{EPRINT:MorYamYam24}} (ucMAC); 
\draw[thick,->] (qqUPSG)  to node [right,midway] {\cite{EPRINT:MorYamYam24}} (SKE+MAC); 
\draw[thick,->] (QPOTP) to [bend left=20] node [below,midway] {\cite{TQC:MorYam24}} (OWSG.east); 
\draw[thick,->] (QPOTP) to [bend left=35] node [right,midway] {\cite{TQC:MorYam24}} (EFI.east);
\draw[very thick,->,dotted] (PrivMon)  to node [left ,midway] {\cite{TQC:MorYam24}}  (OWSG); 
\draw[very thick,->,dotted] (OWSG)     to node [left ,midway] {\cite{STOC:KhuTom24}}  (EFI); 
\draw[thick,->] (PRSG) to node [left,pos=.4] {\cite{C:JiLiuSon18}}  (PrivMon);
\draw[thick,->] (PRSG) to [bend left] node [right,pos=.7] {\cite{C:AnaQiaYue22}} (QPOTP); 
\draw[thick,->] (cqUPSG)  to [bend right] node [left,pos=.25] {\cite{EPRINT:MorYamYam24}} (OWSG); 
%\draw[thin,->] (cqPRFSG) to [bend left] node [right,midway] {\cite{TCC:AGQY22}} (oTCCSKE); 
%
\draw[triv] (PRNRQGA) to node [right,midway] {}  (PRQGA); 
\draw[triv] (PRNRQGA) to node [left ,midway] {}  (UCNRQGA); 
\draw[triv] (PRQGA)   to node [left ,midway] {}  (UCQGA);
\draw[triv] (UCNRQGA) to node [left, midway] {}  (UCQGA);
\draw[triv] (UCNRQGA) to node [left, midway] {}  (UPNRQGA);
\draw[triv] (UCQGA)   to node [left, midway] {}  (UPQGA);
\draw[triv] (UPNRQGA) to node [left, midway] {}  (UPQGA);
% \draw[triv] (PRQGA)   to [bend left] node [right,midway] {} (OWQGA);
% \draw[open] (OWQGA)   to node [right,midway] {} (UPQGA);
% \draw[triv] (UPQGA)   to node [below,midway] {OK} (UPSG);
% \draw[triv] (UPNRQGA) to node [left ,midway] {}  (UPQGA);
% \draw[triv] (UCNRQGA) to node [left, midway] {}  (UCQGA);
% \draw[triv] (UCQGA)   to node [left, midway] {OK}(OWQGA);
% \draw[triv] (UCQGA)   to node [left, midway] {??}(PrivMon); 
%\draw[triv] (UPQGA)   to node [right,midway] {??}(OWQGA);
%
\draw[open] ([yshift=-10pt] cqPRFSG.north east) -- coordinate (m1) ([yshift=0pt] qqPRFSG.south west) node [below,midway] {??}; 
\draw[blue,thick,shift={(m1)}](-0.2,-0.2)--(0.2,+0.2);
\draw[open] ([yshift=-10pt] cqUCFSG.north east) -- coordinate (m2) ([yshift=0pt] qqUCFSG.south west) node [below,midway] {??};
\draw[blue,thick,shift={(m2)}](-0.2,-0.2)--(0.2,+0.2); 
\draw[open] ([yshift=-10pt]  cqUPSG.north east) -- coordinate (m3) ([yshift=0pt]  qqUPSG.south west) node [below,midway] {??};
\draw[blue,thick,shift={(m3)}](-0.2,-0.2)--(0.2,+0.2);
% \draw[thin ,red,->] (MAC)     to node [below,midway] {x?} (ucMAC); 
\draw[ours] (PRDHQGA) to node [right,midway] {\cref{lem:PRetc->NR}}   (PRNRQGA); 
\draw[ours] (PRQGA)   to node [above,midway] {\cref{thm:PR->PRSG}}    (PRSG);
\draw[ours] (UCQGA)   to node [above,pos=.7] {\cref{thm:UC->PrivMon}} (PrivMon);
\draw[ours] (UCQGA)   to node [right,midway] {\cref{lem:UC->OW}}      (OWQGA); %As \cite{TQC:MorYam24}
\draw[ours] (PRNRQGA) to node [above,midway] {\cref{thm:PRNR->PRFSG}} (cqPRFSG);
\draw[ours] (UCNRQGA) to node [above,midway] {\cref{thm:UCNR->UCFSG}} (cqUCFSG); 
\draw[ours] (UPNRQGA) to node [above,midway] {\cref{thm:UPNR->UPFSG}} (cqUPSG);
\draw[ours] (OWQGA)   to node [above,midway] {\cref{thm:OW->OWSG}}    (OWSG);
% \draw[very thick,red,->] (cqUPSG)  to [bend left] node [above,midway] {\cref{thm:cqUPSG_UPQGA}} (-4,0) to (UPQGA);
\end{tikzpicture}
\caption{Relations. ``cq'' and ``qq'' denote classical-query and quantum-query. ``qm'' means that quantum-message. 
A gray dashed arrow from primitive A to primitive B represents that primitive A trivially implies primitive B. 
A dotted arrow from primitive A to primitive B represents that primitive A with pure outputs implies primitive B.
*: \cite{C:AnaQiaYue22} shows that cqPRFSG implies IND-CPA qmSKE. Combined with the relation that cqUPSG implies EUF-CMA MAC, cqPRFSG implies IND-CPA qmSKE + EUF-CMA MAC. 
If the input space is poly, then PRSG implies cqPRFSG~\cite{C:AnaQiaYue22}. 
\xagawa{Q: Is there an arrow from cqMAC to OWSG? Maybe we can do it.}
}
\label{fig:relations}
\end{figure}




% \begin{figure}
% \centering
% \footnotesize
% \begin{tikzpicture}[scale=0.6,%
% triv/.style={thick,draw=black!60,->,dashed},
% open/.style={thick,blue,->},
% ours/.style={very thick,draw=red,->},
% ]
% %
% \node (qqUCFSG) at ( 10,10) {qqUCFSG} ;
% \node (cqUCFSG) at (  5, 9) {cqUCFSG} ;
% \node (qqUPSG)  at ( 10, 7) {qqUPFSG} ;
% \node (cqUPSG)  at (  5, 6) {cqUPFSG} ;
% \node (SKE+MAC) at (7.5, 4) {SKE+cqdMAC} ;
% \node (qqdMAC)  at ( 10, 2) {qqdMAC} ;
% \node (cqdMAC)  at (  5, 1) {cqdMAC} ;
% \node (qqrMAC)  at ( 10,-1) {qqrMAC} ;
% \node (cqrMAC)  at (  5,-2) {cqrMAC} ;
% \node (ucdMAC)  at (  0, 8) {UC dMAC} ;
% \node (ucrMAC)  at ( -5, 5) {UC rMAC} ;
% \node (porMAC)  at (  0, 2) {PO rMAC} ;
% \node (PrivMon) at ( -5,-1) {Private Money} ; 
% %
% \draw[triv] ([yshift=4pt] qqUCFSG.south west) to node [above,midway] {} ([yshift=0pt] cqUCFSG.north east);
% \draw[triv] ([yshift=4pt]  qqUPSG.south west) to node [above,midway] {} ([yshift=0pt]  cqUPSG.north east);
% \draw[triv] (cqUCFSG) to node [above,midway] {} (ucdMAC);
% \draw[triv] (qqUCFSG) to node [above,midway] {} (qqUPSG);
% \draw[triv] (cqUCFSG) to node [above,midway] {} (cqUPSG);
% \draw[triv] (SKE+MAC) to node [right,midway] {} (cqdMAC);
% \draw[triv] (qqUPSG)  to node [left ,midway] {} (qqdMAC);
% \draw[triv] (cqUPSG)  to node [left ,midway] {} (cqdMAC);
% \draw[triv] (qqdMAC)  to node [left ,midway] {} (qqrMAC);
% \draw[triv] (cqdMAC)  to node [left ,midway] {} (cqrMAC);
% \draw[triv] (qqdMAC)  to node [right,midway] {} (cqdMAC);
% \draw[triv] (qqrMAC)  to node [right,midway] {} (cqrMAC);
% %
% \draw[triv] (ucdMAC)  to node [right,midway] {} (cqdMAC);
% \draw[triv] (ucdMAC)  to node [right,midway] {} (porMAC);
% \draw[triv] (ucdMAC)  to node [right,midway] {} (ucrMAC);
% \draw[triv] (ucdMAC)  to node [right,midway] {} (PrivMon);
% \draw[triv] (porMAC)  to node [right,midway] {} (cqrMAC);
% \draw[triv] (ucrMAC)  to [bend left] node [right,midway] {} (cqrMAC);
% %
% \draw[thick,->] (qqUPSG)  to node [right,midway] {\cite{EPRINT:MorYamYam24}} (SKE+MAC); 
% \draw[thick,->] (SKE+MAC) to node [above,midway] {\cite{EPRINT:MorYamYam24}} (porMAC); 
% % 
% \draw[open] (porMAC)   to node [right,midway] {??} (PrivMon);
% \draw[open] (ucrMAC)   to node [right,midway] {??} (PrivMon);
% \draw[open,<->] (ucrMAC)   to node [right,midway] {??} (porMAC);
% % \draw[open] ([yshift=-4pt] cqUCFSG.north east) to node [below,midway] {??}([yshift=0pt] qqUCFSG.south west);
% % \draw[open] ([yshift=-4pt]  cqUPSG.north east) to node [below,midway] {??}([yshift=0pt]  qqUPSG.south west);
% \end{tikzpicture}
% \caption{Relations among quantum-state MACs.
% "po" means "plus-one"-like security that any efficient adversary cannot output valid $t+1$ tags for $m^*$ while it receives $t$ tags for $m^*$. 
% \xagawa{We need to decide which arrows are considered trivial.}
% }
% \label{fig:relations-MAC}
% \end{figure}



==> memo_on_HPSs.tex <==

\section{???}



\begin{itemize}
\item Quantum analogue of Hash Proof System??? It will require $G$ to be a group. 
\item Dual-mode PKE, and OT from group action uses a pairwise independent hash function $H: S^\ell \to \{0,1\}$. Thus, we need to extract 
\end{itemize}

\paragraph{Quantum analogue of HPS:}
Let $(G,S,\star)$ be a PR QGA. 
Let $\ket{\phi_0}$ and $\ket{\phi_1}$ be publicly, efficiently generable elements.
Define the input space $\Sigma$ as 
\[
\Sigma = \{\ket{\psi_0}^{\otimes \ell} \otimes \ket{\psi_1}^{\otimes \ell}:
 \exists (g_0,g_1) \in G \text{ s.t. } \ket{\psi_0} = g_0 \ket{\phi_0}, \ket{\psi_1} = g_1 \ket{\phi_0} \}. 
\]
We also define a subset $L \subseteq \Sigma$ as 
\[
L = \{\ket{\psi_0}^{\otimes \ell} \otimes \ket{\psi_1}^{\otimes \ell}:
 \exists g \in G \text{ s.t. } \ket{\psi_0} = g \ket{\phi_0}, \ket{\psi_1} = g \ket{\phi_0} \}.
\]
Let $K = G^\ell \times \{0,1\}^\ell$. 
We define a hash function $\Lambda$ as 
\[
\Lambda((\myvec{h},\myvec{b}), \ket{\psi_0}^{\otimes \ell} \otimes \ket{\psi_1}^{\otimes \ell})
 = (h_1 \ket{\psi_{b_1}}, \dots, h_\ell \ket{\psi_{b_\ell}}). 
\]
Define a projection $\alpha \colon K \to P$ as 
\[
\alpha((\myvec{h},\myvec{b})) 
 = (h_1 \ket{\phi_{b_1}}, \dots, h_\ell \ket{\phi_{b_\ell}}). 
\]

\begin{itemize}
\item 
Subset membership problem: Let us draw two samples $\sigma_0$ from $L$ and $\sigma_1$ from $\Sigma$. Then, those are computationally indistinguishable. 
\xagawa{We can show it}
\item 
Projective Evaluation: 
For any $(\myvec{h},\myvec{b}) \in K$ and $\sigma = \ket{\psi_0}^{\otimes \ell} \otimes \ket{\psi_1}^{\otimes \ell} \in L$, we have 
$\mathsf{ProjEval}(\alpha((\myvec{h},\myvec{b})), w) = \Lambda((\myvec{h},\myvec{b}), \sigma)$, where $w$ is a member ship witness, that is, $g \in G$. 
\xagawa{Let $(\ket{\xi_1},\dots,\ket{\xi_\ell}) = \alpha((\myvec{h},\myvec{b}))$. 
This property requires \emph{commutativity of $G$} to show $g \ket{\xi_1} = g (h_1 \ket{\phi_{b_1}}) = h_1 (g \ket{\phi_{b_1}}) = h_1 \ket{\psi_{b_1}}$.}

\item Universality. 
If $\sigma \in \Sigma \setminus L$, 
 then $H_{\infty}\big(\Lambda((\myvec{h},\myvec{b}),\sigma) \mid (\alpha((\myvec{h},\myvec{b})),\sigma)\big) \geq \lg(1/\epsilon)$. 
\xagawa{
Let $(\ket{\psi_0},\ket{\psi_1}) = (g_0 \ket{\phi_0}, g_1 \ket{\phi_1})$ with $g_0 \neq g_1$ since they are outside of $L$. 
Let $(\ket{\xi_1},\dots,\ket{\xi_\ell})$ be $\alpha((\myvec{h},\myvec{b})),\sigma)$, 
 which are computed as $\ket{\xi_i} = h_i \ket{\phi_{b_i}}$.  
To show universality with $\lg(1/\epsilon) = \ell$, we will require that there are two $d_{i,0},d_{i,1} \in G$ such that $\ket{\xi_i} = d_{i,0} \ket{\phi_0} = d_{i,1} \ket{\phi_1}$ (and $G$ samples its element uniformly at random). 
If so, $\sigma$ and $\alpha((\myvec{h},\myvec{b}))$ hides information of $b_i$'s. 
By the way, $h_i \ket{\psi_{b_i}} = h_i g_{b_i} \ket{\phi_{b_i}} = g_{b_i} \ket{\xi_i}$. 
Thus, $g_0 \neq g_1$ implies $h_i \ket{\psi_{b_i}}$ has one-bit entropy. 
}

\item To make IND-CPA KEM from HPS; $\alpha((\myvec{h},\myvec{b}))$ should be a public key, 
a ciphertext is $\sigma \gets L$, 
a key is $K = \algo{KDF}(\algo{ProjEval}(\alpha((\myvec{h},\myvec{b})), w))$. 
The decryption computes $\Lambda((\myvec{h},\myvec{b}), \sigma)$. 
\xagawa{In the proof, we will replace $\sigma \in L$ with $\sigma \in \Sigma$. If $\sigma \in \Sigma \setminus L$, then $\algo{ProjEval}(\alpha((\myvec{h},\myvec{b})),w)$ has min-entropy $\ell$. Thus, $K$ is statistically indistinguishable from random. How can we compute $K$ with $\algo{KDF}$???}
\end{itemize}


\paragraph{Quantum analogue of Dual-mode PKE:}

\begin{itemize}
\item Setup with decryption mode: \xagawa{Produce a DDH tuple.}
Let $pp_{dec} = (\ket{\phi_0}, \ket{\phi_1}, t \ket{\phi_0}, t \ket{\phi_1})$ with trapdoor $t$. 
\item Setup with messy mode: \xagawa{Produce a non-DDH tuple.}
Let $pp_{messy} = (\ket{\phi_0}, \ket{\phi_1}, t_0 \ket{\phi_0}, t_1 \ket{\phi_1})$ with trapdoor $(t_0,t_1)$.
\item $Gen(pp = (\ket{\phi_0},\ket{\phi_1},\ket{\psi_0},\ket{\psi_1}), \sigma \in \{0,1\})$:
$\sk = s$ and $\pk = (s \ket{\phi_\sigma}, s \ket{\psi_\sigma})$. 
\item $Enc(\pk = (\ket{\phi},\ket{\psi}),\beta\in\{0,1\},m)$:
For $i \in [\ell]$:
sample $r_i \gets G$ and $b_i \gets \{0,1\}$; 
compute $\ket{c_i} = r_i \ket{\phi_\beta}$ if $b_i = 0$ and $r_i \ket{\psi_\beta}$ if $b_i = 1$; 
compute $\ket{c'_i} = r_i \ket{\phi}$ if $b_i = 0$ and $r_i \ket{\psi}$ if $b_i = 1$. 
Output a ciphertext ct = $\ket{c_1} \otimes \dots \otimes \ket{c_\ell}$ 
 and $H(\ket{c'_1}\otimes \dots \otimes \ket{c'_\ell}) \oplus m$. 
\xagawa{This is a problematic. How can we extract a random string from a quantum state?}
\end{itemize}

\xagawa{This will require \emph{commutativity} also.}

\paragraph{Two-message statistically sender-private OT:}

This uses Dual-mode PKE essentially. 
\begin{itemize}
\item A receiver sends $(\ket{\phi_0},\ket{\phi_1}, \ket{y} = s \ket{\phi_0}, \ket{\psi_0}, \ket{\psi_1})$
 with $\ket{\psi_{\beta}} = s \ket{\phi_1}$ and $\ket{\psi_{1-\beta}} = u \ket{\phi_1}$. 
\xagawa{For $\beta$, we have a DDH tuple
$(\ket{\phi_0},\ket{\phi_1}, \ket{y},\ket{\phi_\beta})$ with a witness $s$. 
For $1-\beta$, we have a non-DDH tuple.
$(\ket{\phi_0},\ket{\phi_1}, \ket{y},\ket{\phi_{1-\beta}})$ with a witness $(s,w)$. 
}
\end{itemize}






==> otherapplications.tex <==
\section{Other Applications}
\mor{remove this section?}
\xagawa{I agree to remove.}
\subsection{Commitments from OW QGAs}
Let $(G,S)$ be a OW QGA.
From it, we construct a commitment scheme as follows.
\begin{align}
Q_0|0...0\rangle&=\frac{1}{\sqrt{|G|^2|S|}}\sum_{g\in G,g_0\in G,s_0\in S}|[g],[g_0],[s_0]\rangle \otimes g|s_0\rangle\\
Q_1|0...0\rangle&=\frac{1}{\sqrt{|G|^2|S|}}\sum_{g\in G, g_0\in G, s_0\in S}|[g],[g_0],[s_0]\rangle \otimes gg_0|s_0\rangle.
\end{align}
Assume that the computational binding is broken.
This means that there exists a polynomial $p$ and a QPT $U$ such that
\begin{align}
\frac{1}{p}&\le
\left|\left(\frac{1}{\sqrt{|G|^2|S|}}\sum_{g\in G,g_0\in G,s_0\in S} \langle [g],[g_0],[s_0]|\otimes \langle s_0|g_0^\dagger g^\dagger \right)   
(I\otimes U)
\left(\frac{1}{\sqrt{|G|^2|S|}}\sum_{g\in G,g_0\in G,s_0\in S} |[g],[g_0],[s_0]\rangle \otimes g|s_0\rangle \right)\right|^2   \\
&\le
\frac{1}{|G|^2|S|}
\sum_{g\in G,g_0\in G,s_0\in S} |\langle s_0|g_0^\dagger g^\dagger U
g|s_0\rangle|^2\label{binding}   
\end{align}
From $U$, we construct a QPT adversary $\cA$ that breaks the OW QGAs as follows.
\begin{enumerate}
    \item 
    Receive $g_0|s_0\rangle$, where $g_0\gets G$ and $s_0\gets S$.
    \item
    Sample $g\gets G$, and returns $g U g^\dagger$.
\end{enumerate}
The probability that $\cA$ wins is equal to \cref{binding},
and therefore $\cA$ breaks the binding.

For statistical hiding, we require that
\begin{align}
\TD\left(
\frac{1}{|G|^2|S|}
\sum_{g\in G,g_0\in G,s_0\in S}
g|s_0\rangle\langle s_0|g^\dagger,
\frac{1}{|G|^2|S|}
\sum_{g\in G,g_0\in G,s_0\in S}
gg_0|s_0\rangle\langle s_0|g_0^\dagger g^\dagger
\right)    
\le\negl(\secp).
\end{align}


\subsection{Quantum Claw-Free Functions}

\cite{C:BraYun90} constructed claw-free functions from OW-GAs.

\begin{definition}[Quantum Claw-Free Functions]
For a unitary $g$, we define two functions $f_0$ and $f_1$ as follows: 
\begin{align}
f_0(g)&=g|s_0\rangle \\   
f_1(g)&=gg_0|s_0\rangle.   
\end{align}
We say that those functions are \emph{claw-free} if for any QPT $\cA$ and any polynomial $t$,
$\Pr[\top\gets\cC]\le\negl(\secp)$, where 
\begin{enumerate}
    \item 
    The challenger $\cC$ chooses $g_0\gets G$ and $|s_0\rangle\gets S$.
    \item 
    $\cC$ sends $|s_0\rangle^{\otimes t}$  and $(g_0|s_0\rangle)^{\otimes t}$ to the adversary $\cA$.
    \item 
    $\cA$ outputs $g_1,g_2$.
    \item 
    $\cC$ projects $g_1|s_0\rangle$ onto $g_2g_0|s_0\rangle$. If the projection is successful,
    $\cC$ outputs $\top$. Otherwise, $\cC$ outputs $\bot$.
\end{enumerate}
\end{definition}

\begin{theorem}
If OW-QGAs exist, then Quantum Claw-Free Functions exist.    
\end{theorem}
\begin{proof}
The reduction algorithm outputs $g = g_2^{-1} g_1$. 
\end{proof}

% If we have claw-free permutations $\{f_0,f_1\}$, then we can construction a collision-resistant hash functions with key $f_0,f_1$ and $s \in S$ as follows: 
% $h_{f_0,f_1,I}(w) = f_{w_0}(f_{w_1}(\cdots f_{w_{|w|}}(s) \cdots ))$. 
% But, we cannot use QCFF to construction collision-free functions. 
% % Suppose that the adversary outputs two strings $w$ and $w'$ of length $\ell$ and $\ell'$. (We need prefix-free encoding.)
% % If $w_1 = w'_1$, then we have a claw. Otherwise, we have 
% % $f_{w_2}(\cdots f_{w_\ell}(s) \cdots ) = f_{w'_2}(\cdots f_{w_{\ell'}}(s) \cdots )$. 



\subsection{}
Other applications?
Hash proof system~\cite{AC:ADMP20}
\cite{AC:ADMP20}'s PKE has quantum pk, so maybe not interesting.
\cite{AC:ADMP20} construct OT. 
\cite{TCC:JQSY19} construct identification and digital signatures.
Why do they directly construct identification and DS from GA, although one-way GA gives OWF? 
\xagawa{DS from GA has no limitation of queries because it is constructed from Unruh/FS transforms.}
\cite{TCC:JQSY19} also construct bit commitment. OWSGs imply bit commitment. Is there any advantage?
\cite{C:BraYun90} construct bit commitment that has the special property that two the same commitments can be convinced without revealing bits,
and trapdoor property that means that the binding can be broken by using the trapdoor.

\subsection{Weak PRUs}
\begin{definition}[Weak PRUs]
For any polynomial $Q$,
$\{|x_q\rangle,U_k|x_q\rangle\}_{q\in[Q]}$
and 
$\{|x_q\rangle,U|x_q\rangle\}_{q\in[Q]}$
are computationally indistinguishable.
Here, $|x_q\rangle\gets S$, $k\gets\bit^\kappa$, and $U\gets\mu$.
\end{definition}

